A Bregman Learning Framework for Sparse Neural Networks

We propose a learning framework based on stochastic Bregman iterations, also known as mirror descent, to train sparse neural networks with an inverse scale space approach. We derive a baseline algorithm called LinBreg, an accelerated version using momentum, and AdaBreg, which is a Bregmanized generalization of the Adam algorithm. In contrast to established methods for sparse training the proposed family of algorithms constitutes a regrowth strategy for neural networks that is solely optimization-based without additional heuristics. Our Bregman learning framework starts the training with very few initial parameters, successively adding only significant ones to obtain a sparse and expressive network. The proposed approach is extremely easy and efficient, yet supported by the rich mathematical theory of inverse scale space methods. We derive a statistically profound sparse parameter initialization strategy and provide a rigorous stochastic convergence analysis of the loss decay and additional convergence proofs in the convex regime. Using only 3.4% of the parameters of ResNet-18 we achieve 90.2% test accuracy on CIFAR-10, compared to 93.6% using the dense network. Our algorithm also unveils an autoencoder architecture for a denoising task. The proposed framework also has a huge potential for integrating sparse backpropagation and resource-friendly training.

==> Bregmanized Training of Sparse Neural Networks/commands.tex <==
% comment functions
\newcommand{\lb}[1]{{\color{red}#1}}
\newcommand{\mb}[1]{{\color{purple}#1}}

\definecolor{internationalkleinblue}{rgb}{0.0, 0.18, 0.65}
\newcommand{\tr}[1]{{\color{internationalkleinblue}#1}}
\newcommand{\revision}[1]{{\color{magenta}#1}}
\renewcommand{\revision}[1]{#1}

\newcommand{\comment}[1]{}

% general math
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\lip}{\operatorname{Lip}}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\prox}[1]{\,\mathrm{prox}_{#1}}
\newcommand{\abs}[1]{\left\vert#1\right\vert}
\newcommand{\norm}[1]{\Vert#1\Vert}
\newcommand{\st}{\,:\,}
\DeclareMathOperator*{\Lip}{Lip}
\DeclareMathOperator*{\sign}{sign}
\newcommand{\eps}{\varepsilon}
\DeclareMathOperator{\dom}{dom}

% specific
\newcommand{\param}{\theta}
\newcommand{\weight}{W}
\newcommand{\bias}{b}
\newcommand{\net}{f}     %{\mathcal{N}}
\newcommand{\inp}{x}
\newcommand{\inpp}{x'}
\newcommand{\oup}{y}
\newcommand{\oupp}{y'}
\newcommand{\Inp}{\mathcal{X}}
\newcommand{\Oup}{\mathcal{Y}}
\newcommand{\Param}{\Theta}
\newcommand{\noTr}{K}
\newcommand{\trSet}{\mathcal{T}}
\newcommand{\trSetY}{\mathcal{T}_\Oup}
\newcommand{\loss}{\ell}
\newcommand{\empBatchLoss}{L}
\newcommand{\empLoss}{\mathcal{L}}
\newcommand{\popRisk}{\mathcal{R}}
\newcommand{\relu}{\operatorname{ReLU}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\V}{\mathbb{V}}
\newcommand{\Exp}[1]{\E\left[#1\right]}
\newcommand{\Var}[1]{\mathrm{Var}\left[#1\right]}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\func}{J}
\newcommand{\sg}{p}
\newcommand{\regParam}{\alpha}
\newcommand{\timeStep}{\tau}
\newcommand{\tol}{\mathrm{tol}}
\newcommand{\acc}{\mathcal{A}(\net_\param)}
\renewcommand{\d}{\mathrm{d}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\LinBreg}{\mbox{LinBreg}}
\newcommand{\AdaBreg}{\mbox{AdaBreg}}

%environments
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{cor}[theorem]{Corollary}
\newtheorem{assumption}{Assumption}
% \newtheorem{example}[theorem]{Example}
% \theoremstyle{remark}
% \newtheorem{remark}[theorem]{Remark}

%equation numbering
\numberwithin{equation}{section}


==> Bregmanized Training of Sparse Neural Networks/packages.tex <==
\usepackage[utf8]{inputenc}

%
% \usepackage{graphicx}
% Used for displaying a sample figure. If possible, figure files should
% be included in EPS format.
%
% If you use the hyperref package, please uncomment the following line
% to display URLs in blue roman font according to Springer's eBook style:
% \renewcommand\UrlFont{\color{blue}\rmfamily}

%graphics
\usepackage{graphicx}

%color
\usepackage{color}

%bibliography
% \usepackage[
% natbib,
% maxcitenames=3, 
% maxbibnames=10,  
% sorting=ydnt,
% sortcites,
% defernumbers,
% backend=biber
% ]{biblatex}
% \addbibresource{bibliography.bib}

%hyperref
\usepackage{hyperref}
\hypersetup{
	%colorlinks = true,
    final=true, 
    plainpages=false,
    pdfstartview=FitV,
    pdftoolbar=true,
    pdfmenubar=true,
    pdfencoding=auto,
    psdextra,
    bookmarksopen=true,
    bookmarksnumbered=true,
    breaklinks=true,
    linktocpage=true,
    %urlcolor=blue,
 	%citecolor=blue,
 	%linkcolor=blue,
 	pdfinfo={
 	    Title={A Bregman Learning Framework for Sparse Neural Networks},
	    Keywords={Bregman Iterations, Sparse Neural Networks, Inverse Scale Space, Optimization}
	    author={Leon Bungert, Tim Roith, Daniel Tenbrinck, Martin Burger}}
}
%math
\usepackage{amssymb,amsmath}


%algorithm
\usepackage[ruled,vlined]{algorithm2e}
\usepackage{setspace}

%ref
\usepackage[capitalise,noabbrev,nameinlink]{cleveref}
\crefname{assumption}{Assumption}{Assumptions}
\newcommand{\crefrangeconjunction}{--}

\crefname{example}{Example}{Examples}
\crefname{lemma}{Lemma}{Lemmata}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{proposition}{Proposition}{Propositions}
\crefname{remark}{Remark}{Remarks}
\crefname{definition}{Definition}{Definitions}

%tables
\usepackage{booktabs}
\usepackage{multirow}

%figures
\usepackage{caption}
\usepackage{subcaption}

%MISC
\usepackage{enumitem}
\usepackage[margin=1.5in]{geometry}
\usepackage{hhline}
\usepackage{todonotes}
\setuptodonotes{inline}

\setlength{\parskip}{0pt}

\usepackage{tabularx}
\newcolumntype{R}{>{\raggedright\arraybackslash}X}
\newcolumntype{C}{>{\centering\arraybackslash}X}
\newcolumntype{L}{>{\raggedleft\arraybackslash}X}
